Greedy Algorithm for Structured Bandits: A Sharp Characterization of Asymptotic Success / Failure

We study the greedy (exploitation-only) algorithm in bandit problems with a known reward structure. We allow arbitrary finite reward structures, while prior work focused on a few specific ones. We fully characterize when the greedy algorithm asymptotically succeeds or fails, in the sense of sublinear vs. linear regret as a function of time. Our characterization identifies a partial identifiability property of the problem instance as the necessary and sufficient condition for the asymptotic success. Notably, once this property holds, the problem becomes easy -- any algorithm will succeed (in the same sense as above), provided it satisfies a mild non-degeneracy condition. Our characterization extends to contextual bandits and interactive decision-making with arbitrary feedback. Examples demonstrating broad applicability and extensions to infinite reward structures are provided.

==> app-extensions.tex <==
\section{[OBSOLETE!] Extensions to Infinite Function Classes}

\begin{definition}[$\eps$-interior reward function]\label{def:interior} A reward-function $f\in\cF$ is called \emph{$\eps$-interior} with respect to $\cF$ if its $\eps$-neighborhood $\{f':\|f'-f\|_2\le\eps\}$ is a subset of $\cF$. %If this $f$ is a decoy for another reward function $f'$, then we call $f$ an \emph{$\eps$-interior decoy} of $f'$.
\end{definition}

We note that the choice of $L_2$ distance is not essential in Definition~\ref{def:interior}; any $L_p$ distance suffices.

%one can relax the $\{f':\|f'-f\|_2\le\eps\}$ in Definition~\ref{def:interior} to $\{f':f'(a)=f(a)+\eps'\ind{a=\arg\max f}\}$

%\begin{definition}[$\eps$-interior decoy] Let $f^*,f\dec$ be two reward functions. Call $f\dec$ an \emph{$\eps$-interior decoy} for $f^*$ if $f\dec$ an \emph{$\eps$-interior decoy} for $f^*$.\end{definition}

We show that Theorem~\ref{thm:MAB}(b) can be seamlessly extended to infinite $\cF$, with the requirement $f\dec\in\cF$ being strengthened to $f\dec$ being $\eps$-interior ($\eps>0$). In other words, existence of \emph{$\eps$-interior decoy} implies failure of \Greedy in infinite function classes.

\begin{theorem}\label{thm:infinite-failure}
    Fix a problem instance $(f^*,\cF)$ of \StructuredMAB. Suppose the warm-up data consists of one sample for each arm. Assume $f^*$ has a decoy $f\dec$ {\color{blue}that is $\eps$-interior with respect to $\cF$ for some $\eps>0$}, with decoy arm $a\dec$. Then with some probability $p\dec>0$ it holds that \Greedy chooses $a\dec$ for all rounds $t\in (T_0, \infty)$. We can lower-bound $p\dec$ by
$\color{blue}e^{-O(K/\eps^2)}$.
\end{theorem}

Compared to Theorem~\ref{thm:MAB}(b), the failure probability $p\dec$ in Theorem~\ref{thm:infinite-failure} does not depend on the function-gap $\Gamma(f\dec)$ (which can easily be 0 for an infinite $\cF$) at all, but depends on $\eps>0$ instead. Theorem~\ref{thm:infinite-failure} marks a promising direction: the requirement of a positive function-gap (natural for  discrete function classes) can be removed for continuous function classes as long as the decoy does not lie in the ``boundary'' of $\cF$. We expect similar results to hold for contextual bandits and general interactive decision-making as well.

%For any $\eps>0$, define $\cF_{\eps}:=\{f':\|f'-f\|_1\le\eps, f\in\mathcal{F}\}$.

The proof of Theorem~\ref{thm:infinite-failure} follows the same template as the proof of Theorem~\ref{thm:MAB}(b) (see Appendix~\ref{sec:mabFailure}), with a crucial difference: although we still want to show that \Greedy will get stuck in $a\dec$ permanently (with constant probability), we must admit the fact that the outputs of the least-squares regression oracle may ``fluctuate'' around $f\dec$ over time (due to randomness of rewards and the nature of continuous function classes) --- we cannot prove $f\dec$ is always chosen by the regression oracle any more. The key insight of our new proof is that although the outputs of the regression oracle fluctuate, the fluctuation does not affect the downstream (greedy) decision $a\dec$. In other words, small fluctuation in prediction does not translate to decision-making (with constant probability).

We now present our proof. To begin with, define
\begin{align*}
E_1 = \cbr{ \abs{\AveRewWarmUp(a) - f\dec(a)} < \eps/(2\sqrt{K})
\quad\text{for each arm $a\neq a\dec$}},
\end{align*}
\begin{align*}
E_2 = \cbr{ \forall t>T_0,\; \abs{\bar{r}_t(a\dec) - f^*(a\dec)}  \le \eps / (2\sqrt{K})},
\end{align*}
which are similar to \eqref{eq:MAB-neg-pf-E1} and \eqref{eq:MAB-neg-pf-E2} in the proof of Theorem~\ref{thm:MAB}(b), with the only difference of replacing $\Gamma(f\dec)/2$ by $\eps/(2\sqrt{K})$. Changing the notation immediately yields replacements of Lemmas \ref{lm:E1}, \ref{lm:E2}, and \ref{lm:intersection} below, with no change in the proof beyond notation.

\begin{lemma}
Event $E_1$ happens with probability at least $\left[ \frac{\eps}{\sqrt{2\pi\sigma^2K}} \exp(- 2 / \sigma^2 ) \right]^{K-1}$.
\end{lemma}


\begin{lemma}
For some appropriately chosen $\sigma = \Theta(\eps/\sqrt{K})$, we have event $E_2$ happens with probability at least
\[
\Pr{E_2} \ge 0.9.
\]
\end{lemma}

\begin{lemma}
For some appropriately chosen $\sigma = \Theta(\eps/\sqrt{K})$, we have the following lower bound:
\[
\Pr[E_1\cap E_2] \ge \left[ \Omega(\exp(-2/\sigma^2)) \right]^{K-1}
\]
\end{lemma}
\begin{proof}
Note that event $E_1$ and $E_2$ are independent, then, the probability of $E_1\cap E_2$ can be obtained from the previous two lemmas.
\end{proof}

We now prove a crucial lemma which is an extension of Lemma~\ref{lm:stuck} to the infinite $\cF$ setting.

\begin{lemma}\label{lm:infinite-stuck}
Assume event $E_1$ and $E_2$ holds, then greedy algorithm only choose the decoy arm $a\dec$.
\end{lemma}
\begin{proof}{\color{red}To be finished soon.}
% The proof is by induction. Assume by round $t$, the algorithm have only choose the decoy arm $a\dec$. Note that assuming event $E_1$ and $E_2$ holds, for any reward vector $f\neq f\dec$, we will have
% \[
% \abs{\bar{r}_t(a) - f\dec(a)} \le \abs{\bar{r}_t(a) - f(a)},
% \]
% with at least one inequality strict for one arm. Hence $f\dec$ must (still) be the $\MSE_t(\cdot)$ minimizer, and $a\dec$ will be chosen in the next round.
\end{proof}

\Cref{thm:infinite-failure} directly from the above lemmas. 
